Tight Generalization Bounds for Large-Margin Halfspaces

We prove the first generalization bound for large-margin halfspaces that is asymptotically tight in the tradeoff between the margin, the fraction of training points with the given margin, the failure probability and the number of training points.

==> lower.tex <==
\section{Lower Bound}
We define a data distribution $\cD$ over $\R^d$ for sufficiently large $d$. Construct sets of points $X_1,\dots,X_k$ for a parameter $k$ to be determined, such that $X_i$ has cardinality $2^i \tau_i^{-1}$. The data distribution is uniform over $\cup_i X_i$, and the label is always $1$. Note that the total number of points in the support of the distribution is $m=\sum_{i=1}^k 2^i \tau_i^{-1}$. 

The first $k$ coordinates of a point $x$ are chosen so that $x_i = 2^{-(i+3)/2}$. The next $m$ coordinates are chosen so that each of the $m$ points in $\cup_i X_i$ has its own designated coordinate. The coordinate of an $x \in \cup_i X_i$ corresponding to $x$ itself is set to $1/\sqrt{2}$ and all remaining are set to $0$.

The norm of any point $x \in \cup_i X_i$ is $\sqrt{1/2 + \sum_{i=1}^k 2^{-(i+3)}} \leq \sqrt{1/2 + 1/2} = 1$.

Define $\gamma_i := 2^{-(i+4)/2}$. We will now show that for any $X_i$ and any set $T \subseteq X_i$ of $2^i$ points, there is a unit vector $w \in \R^d$ with $\langle w, x\rangle \geq \gamma_i$ for all $x \notin T$ and for all $x \in T$ it holds that $\langle w, x \rangle < 0$.

To see this, let $w$ have $w_i = 1/\sqrt{2}$ and $w_j = 0$ for $j \in \{1,\dots,k\} \setminus \{i\}$. For every point $x \in T$, let the coordinate of $w$ corresponding to $x$ be $-1/\sqrt{2^{i+1}}$. Then $\|w\| = \sqrt{1/2 + |T|/2^{i+1}} = \sqrt{1/2 + 1/2}=1$. We see that for $x \notin T$, we have $\langle w, x\rangle = 2^{-1/2} 2^{-(i+3)/2} = 2^{-(i+4)/2} = \gamma_i$, where the contribution to the inner product comes from the first $k$ coordinates. For $x \in T$, the inner product is instead $2^{-1/2} 2^{-(i+3)/2} - 2^{-(i+1)/2} 2^{-1/2} = 2^{-(i+4)/3}-2^{-(i+2)/2} < 0$.

From the above, we see that the hyperplane corresponding to $w$ has margin at least $\gamma_i$ on all points outside $T$ and it is incorrect on all points in $T$. It follows that $\Loss_{\cD}(w) = |T|/m = \tau_i$.

We will now argue that with constant probability over a training set $\rS \sim \cD^n$, we can choose an $X_i$ and set $T \subset X_i$ with $|T|=2^i$ to assign the label $-1$, such that the corresponding vector $w$ has $\Loss^{\gamma_i}_{\rS}(w)$ significantly smaller than $\tau_i$, creating a gap between $\Loss^{\gamma_i}_{\rS}(w)$ and $\Loss_\cD(w)$.




